Shape-from-Template with Generalised Camera

This article presents a new method for non-rigidly registering a 3D shape to 2D keypoints observed by a constellation of multiple cameras. Non-rigid registration of a 3D shape to observed 2D keypoints, i.e., Shape-from-Template (SfT), has been widely studied using single images, but SfT with information from multiple-cameras jointly opens new directions for extending the scope of known use-cases such as 3D shape registration in medical imaging and registration from hand-held cameras, to name a few. We represent such multi-camera setup with the generalised camera model; therefore any collection of perspective or orthographic cameras observing any deforming object can be registered. We propose multiple approaches for such SfT: the first approach where the corresponded keypoints lie on a direction vector from a known 3D point in space, the second approach where the corresponded keypoints lie on a direction vector from an unknown 3D point in space but with known orientation w.r.t some local reference frame, and a third approach where, apart from correspondences, the silhouette of the imaged object is also known. Together, these form the first set of solutions to the SfT problem with generalised cameras. The key idea behind SfT with generalised camera is the improved reconstruction accuracy from estimating deformed shape while utilising the additional information from the mutual constraints between multiple views of a deformed object. The correspondence-based approaches are solved with convex programming while the silhouette-based approach is an iterative refinement of the results from the convex solutions. We demonstrate the accuracy of our proposed methods on many synthetic and real data

==> backup.tex <==

\subsection{Notation}
Let a volumetric Statistical Shape Model (SSM) be represented by a 3D mean pointcloud of $N$ points denoted by $\bar{\mathbf{P}} \in \mathbb{R}^{3 \times N}$ and the basis pointcloud $\mathbf{P}_{i} \in \mathbb{R}^{3 \times N} \quad \forall i \in [1,M]$, where we have $M$ basis shapes. Therefore any shape can be represented as:
\begin{equation}
    \mathbf{V} = \bar{\mathbf{P}} + \sum_{i=1}^M w_i \mathbf{P}_{i},
\end{equation}
where $w_i$ are the basis weights. The resulting shape can be rotated to any configuration with a rotation $\mathbf{R} \in \mathbb{SO}(3)$, we assume that translation either does not exist or has been suitably accounted for by centering the shape model in the target/viewing configuration. We assume that there are two X-ray cameras which are imaging this shape, the center of these two cameras are at $\mathbf{C}_1, \mathbf{C}_2 \in \mathbb{R}^{3}$, such that $\mathbf{C}_2 = {}^{C_2}\mathbf{R}_{C_1} \mathbf{C}_1 + {}^{C_2}\mathbf{t}_{C_1}$ and $({}^{C_2}\mathbf{R}_{C_1} , {}^{C_2}\mathbf{t}_{C_1})$ are known extrinsics. 

We assume that $(\mathbf{C}_1, \mathbf{C}_2)$ casts a total of $(Q, R)$ rays through $\mathbf{V}$ which forms two X-ray images $(\mathcal{I}_1, \mathcal{I}_2)$. These set of rays are given by $\{L_{1,q}, \forall q \in [1,Q]\}$ and $\{L_{2,r}, \forall r \in [1,R]\}$ for the cameras $\mathbf{C}_1$ and $\mathbf{C}_2$ (resp.). Each ray is defined by the tuple $(\mathbf{C}_1, \mathbf{d}_{1,q})$ and $(\mathbf{C}_2, \mathbf{d}_{2,r})$ for $\mathbf{C}_1$, $\mathbf{C}_2$ resp., where $\mathbf{d}_{1,q}, \mathbf{d}_{2,r} \in \mathbb{S}^2, \forall q, r$. For the $q$-th and $r$-th sightline, we denote the image formation model as:
\begin{equation}
\label{eqn_img_basic}
    \mathcal{I}_{1,q} = \sum_{j=1}^N e^{-\frac{1}{\sigma^2} \big(d(\mathbf{R}\mathbf{V}_j, L_{1,q})\big)^2}, \quad \text{and} \quad \mathcal{I}_{2,r} = \sum_{j=1}^N e^{-\frac{1}{\sigma^2} \big(d(\mathbf{R}\mathbf{V}_j, L_{2,r})\big)^2},
\end{equation}

\noindent where $d(\cdot, \cdot) \in [0,1]$ gives the normalized distance between a point and a line and $\sigma \in [0,2]$ is a weight. By doing a Taylor series expansion of \cref{eqn_img_basic} and ignoring all terms higher than quadratic, we get:
\begin{equation}
    \begin{gathered}
    \label{eqn_img_taylor}
        \mathcal{I}_{1,q} = N - \frac{1}{\sigma^2} \sum_{j=1}^N  \big(d(\mathbf{R}\mathbf{V}_j, L_{1,q})\big)^2, \quad \text{and}\\ 
        \quad \mathcal{I}_{2,r} = N -    \frac{1}{\sigma^2} \sum_{j=1}^N \big(d(\mathbf{R}\mathbf{V}_j, L_{2,r})\big)^2.
    \end{gathered}
\end{equation}
We would like the above expressions in \cref{eqn_img_taylor} to evaluate to a positive value, i.e.,
\begin{equation}
    \begin{gathered}
        N - \frac{1}{\sigma^2} \sum_{j=1}^N  \big(d(\mathbf{R}\mathbf{V}_j, L_{1,q})\big)^2 \geq 0, \quad \text{and} \quad N -    \frac{1}{\sigma^2} \sum_{j=1}^N \big(d(\mathbf{R}\mathbf{V}_j, L_{2,r})\big)^2 \geq 0 \\
        \Rightarrow \sigma^2 \geq \frac{\sum_{j=1}^N  \big(d(\mathbf{R}\mathbf{V}_j, L_{1,q})\big)^2}{N} \leq 1, \quad \text{and} \quad \Rightarrow \quad \sigma^2 \geq \frac{\sum_{j=1}^N \big(d(\mathbf{R}\mathbf{V}_j, L_{2,r})\big)^2}{N} \leq 1. 
    \end{gathered}
\end{equation}
\noindent Therefore, we may claim $\sigma^2 > 1$ as a sufficient condition for ensuring positive values in $(\mathcal{I}_{1,q}, \mathcal{I}_{2,r})~\forall (q,r)$. The point to line distance function from the $j$-th point to the $q$-th or $r$-th line can be written as:
\begin{equation}
\begin{gathered}
        d(\mathbf{R}\mathbf{V}_j, L_{1,q}) = \frac{1}{\Delta} \|(\mathbf{R}\mathbf{V}_j - \mathbf{C}_1 + \langle \mathbf{C}_1 - \mathbf{R}\mathbf{V}_j, \mathbf{d}_{1,q}\rangle \mathbf{d}_{1,q} )\|_2, \quad \text{and}, \\ d(\mathbf{R}\mathbf{V}_j, L_{2,r}) = \frac{1}{\Delta} \|(\mathbf{R}\mathbf{V}_j - \mathbf{C}_2 + \langle \mathbf{C}_2 - \mathbf{R}\mathbf{V}_j, \mathbf{d}_{2,r}\rangle \mathbf{d}_{2,r} )\|_2,
        \label{eqn_dist_func}
\end{gathered}
\end{equation}

\noindent where $\Delta$ is the largest diagonal of the most voluminous basis of the SSM. Given that our unknowns are the 9 elements of rotation matrix $\mathbf{R}$ and the basis weights $\{w_i\}$, $\mathbf{R}\mathbf{V}_j$ is quadratic and therefore, $\mathcal{I}_{1,q}$ and $\mathcal{I}_{2,r}$ must be quartic polynomials.

\subsection{SSM based reconstruction problem}
For two observed images $\hat{\mathcal{I}}_1$ and $\hat{\mathcal{I}}_2$, the reconstruction problem can be written as:
\begin{equation}
    \begin{gathered}
        \min_{\mathbf{R}, \{w_i\}} \| \hat{\mathcal{I}}_{1} - \mathcal{I}_{1} \|_2^2 + \| \hat{\mathcal{I}}_{2} - \mathcal{I}_{2} \|_2^2 \\
        \Rightarrow \min_{\mathbf{R}, \{w_i\}} C(\mathcal{I}_{1}) + C(\mathcal{I}_{2}) \\
        \label{eqn_prblm_stmt}
    \end{gathered}
\end{equation}
Hereafter, we show a series of simplification of the cost-function for the first image $C(\mathcal{I}_{1})$ which generalises well to all images. First, we describe a method to convexly initialize the SSM with a semi-rigid assumption, i.e., when $M=1$. 

\subsubsection{Semi-rigid initialization}

We first expand \cref{eqn_dist_func} for the first camera:
\begin{equation}
    \begin{gathered}
    \label{eqn_long_expr_1}
        d(\mathbf{R}\mathbf{V}_j, L_{1,q}) = \frac{1}{\Delta} \|(\mathbf{R}\mathbf{V}_j - \mathbf{C}_1 + \langle \mathbf{C}_1 - \mathbf{R}\mathbf{V}_j, \mathbf{d}_{1,q}\rangle \mathbf{d}_{1,q} )\|_2 \\
         = \frac{1}{\Delta}\| \begin{bmatrix} \big((\mathbf{d}_{1,q} \mathbf{d}_{1,q}^{\top} - \mathbbm{1}_3) \otimes \mathbf{1}_{1 \times 3} \big) \begin{bmatrix}
             \mathbbm{1}_9 & \mathbbm{1}_9
         \end{bmatrix} & (\mathbf{d}_{1,q} \mathbf{d}_{1,q}^{\top} - \mathbbm{1}_3) \mathbf{C}_1 \end{bmatrix} \mathrm{diag}\Big(\begin{bmatrix}
             \mathbf{1}_{1 \times 3} \otimes \mathbf{P}_{j,1}^{\top} & \mathbf{1}_{1 \times 3} \otimes \tilde{\mathbf{P}}_j^{\top} &1
         \end{bmatrix}\Big) \begin{bmatrix}
             w_1 \mathrm{vec}(\mathbf{R}) \\ \mathrm{vec}(\mathbf{R}) \\ - 1
         \end{bmatrix} \|_2  
    \end{gathered}
\end{equation}

\noindent where $\mathrm{vec}(\mathbf{R}) = (r_{1,1} , r_{1,2} , \hdots, r_{3,3})^{\top}$. We introduce the substitution $w_1 \mathrm{vec}(\mathbf{R}) = (k_{1,1} , k_{1,2} , \hdots, k_{3,3})^{\top}$ and a combined variable for the parameters $\xi = (w_1 \mathrm{vec}(\mathbf{R})^{\top}, \mathrm{vec}(\mathbf{R})^{\top})^{\top} = (k_{1,1} , \hdots, k_{3,3}, r_{1,1}, \hdots, r_{3,3}, 1)^{\top}$. Using the matrices $\mathbf{D}_{j,q,1}$ and $\mathbf{D}_{j,r,2}$ for the data terms in \cref{eqn_dist_func} and in the expression in \cref{eqn_long_expr_1}, we can write:
\begin{equation}
    d(\mathbf{R}\mathbf{V}_j, L_{1,q}) = \frac{1}{\Delta}\|\mathbf{D}_{j,q,1} \xi\|_2, \quad \text{and} \quad d(\mathbf{R}\mathbf{V}_j, L_{2,r}) = \frac{1}{\Delta}\|\mathbf{D}_{j,r,2} \xi\|_2
\end{equation}

\noindent For the $q$-th and $r$-th sightline, the linearised image formation model writes as:
\begin{equation}
    \begin{gathered}
    \label{eqn_img_taylor_simple}
        \mathcal{I}_{1,q} = N - \frac{1}{( \sigma \Delta)^2}\sum_{j=1}^N  \xi^{\top} \mathbf{D}_{j,q,1}^{\top} \mathbf{D}_{j,q,1} \xi, \quad \text{and}\\ 
        \quad \mathcal{I}_{2,r} = N - \frac{1}{( \sigma \Delta)^2}\sum_{j=1}^N  \xi^{\top} \mathbf{D}_{j,r,2}^{\top} \mathbf{D}_{j,r,2} \xi  .
    \end{gathered}
\end{equation}

\noindent We rename $\mathbf{D}_{j,x,y}^{\top} \mathbf{D}_{j,x,y}$ as the projection matrix $\mathbf{M}_{j,x,y}$ and the scaled values $\frac{\mathbf{D}_{j,x,y}^{\top} \mathbf{D}_{j,x,y}}{( \sigma \Delta)^2}$ as the scaled projection matrix $\tilde{\mathbf{M}}_{j,x,y}$. The cost functions are therefore:
\begin{equation}
    \begin{gathered}
    \label{semi_rigid_costs}
        C(\mathcal{I}_{1}) = \sum_{q = 1}^Q \bigg| \hat{\mathcal{I}}_{1,q} - \Big( N - \sum_{j=1}^N  \xi^{\top} \tilde{\mathbf{M}}_{j,q,1} \xi  \Big) \bigg|, \quad \text{and} \\
        C(\mathcal{I}_{2}) = \sum_{r = 1}^R \bigg| \hat{\mathcal{I}}_{2,r} - \Big( N -  \sum_{j=1}^N  \xi^{\top} \tilde{\mathbf{M}}_{j,r,2} \xi  \Big) \bigg|
    \end{gathered}
\end{equation}

\subsubsection{Generalizing to all bases}
We can generalize \cref{eqn_long_expr_1} as follows:

\begin{equation}
    \begin{gathered}
    \label{eqn_long_expr_1}
        d(\mathbf{R}\mathbf{V}_j, L_{1,q}) = \frac{1}{\Delta} \|(\mathbf{R}\mathbf{V}_j - \mathbf{C}_1 + \langle \mathbf{C}_1 - \mathbf{R}\mathbf{V}_j, \mathbf{d}_{1,q}\rangle \mathbf{d}_{1,q} )\|_2 \\
         = \frac{1}{\Delta}\left\lVert \begin{bmatrix} \big((\mathbf{d}_{1,q} \mathbf{d}_{1,q}^{\top} - \mathbbm{1}_3) \otimes \mathbf{1}_{1 \times 3} \big) 
             \big( \mathbf{1}_{1 \times M} \otimes \mathbbm{1}_9 \big)  & (\mathbf{d}_{1,q} \mathbf{d}_{1,q}^{\top} - \mathbbm{1}_3) \mathbf{C}_1 \end{bmatrix} \mathrm{diag}\Bigg(\begin{bmatrix}
             (\mathbf{1}_{1 \times 3} \otimes \mathbf{P}_{j,1}^{\top})^{\top} \\ \vdots \\ (\mathbf{1}_{1 \times 3} \otimes \mathbf{P}_{j,M}^{\top})^{\top} \\ (\mathbf{1}_{1 \times 3} \otimes \tilde{\mathbf{P}}_j^{\top})^{\top} \\ 1
         \end{bmatrix}^{\top}\Bigg) \begin{bmatrix}
             w_1 \mathrm{vec}(\mathbf{R}) \\ \vdots \\ w_M \mathrm{vec}(\mathbf{R}) \\ \mathrm{vec}(\mathbf{R}) \\ - 1
         \end{bmatrix} \right\rVert_2  
    \end{gathered}
\end{equation}


% \noindent \textcolor{red}{Open questions:
% \begin{itemize}
%     \item Is \cref{semi_rigid_costs} convex, assuming the Gram matrix $\xi \xi^{\top}$ is the parameter (given the abs of affine function of a Gram matrix)?
%     \begin{itemize}
%         \item Yes
%     \end{itemize}
%     \item Check sanity of computation, there might very well be some mistakes
%        \begin{itemize}
%         \item Nope
%     \end{itemize}
% \end{itemize}}

+++++++++++++++++++

\vspace{5mm}
\vspace{5mm}
Three dimensional representation offers tremendous advantage over two dimensional ones, when it comes to human visual interpretation of complicated data \citep{tory2004human, dubel20142d}. In a clinical setting, where experts need to observe and analyse complex human anatomies in a time constrained environment, it makes natural sense to try and harness the modern advances in engineering to reconstruct and visualise 3D structures in the best possible manner. To this end, medical imaging researchers have been diligently pursuing novel methods to push the boundaries of 3D reconstruction using data available from existing and new imaging modalities. A common pursuit of clinicians is the non-invasive imaging of human internal organs. X-rays, CT  and MRI scanners form some of the most commonly used imaging modalities. However, all these methods have their pros and cons, necessitating clinicians to go back and forth between these imaging techniques. While CT and MRI scanners, in theory, could always generate accurate 3D reconstructions, it is not always practically feasible. Physical, medical and financial considerations often prevent clinicians from freely choosing the best possible imaging method for a given diagnosis. But ideally, we would like the medical experts to have access to high resolution and accurate 3D reconstructions in all cases, irrespective of practical constraints. This gives rise to the necessity of finding newer directions for reconstruction from diverse imaging techniques, wherein the data may suffer from being sparse, inaccurate, or insufficient in some manner.
\begin{itemize}
    \item \textbf{ToDo:} Introduce geometric methods outside of medical imaging and highlight some of their drawbacks
\end{itemize}
The standard method for 3D reconstruction of human anatomical features are either CT or MRI scan. In our current research, we investigate an alternative imaging modality, biplanar X-ray images, for automatic, globally optimal reconstruction of musculo-skeletal structures.

MRI and CT scanners, despite being highly accurate, suffers some well-known drawbacks. MRI scanners lack adequate portability and poses safety hazards for patients with implants, external devices and accessory medical devices due to the strong magnetic field it generates. CT scans subject patients to a high dosage of radiation due to repeated scans with X-rays. Large-scale surveys have highlighted an `inordinately (sic) increase in cancer risks' \citep{cao2022ct} from CT scans. Biplanar X-rays, on the other hand, work by simultaneously imaging anteroposterior and lateral views of the object to be reconstructed \citep{melhem2016eos}. Imaging from just two views in this biplanar setup, therefore, offer an attractive alternative to CT and MRI scans because: a) they are less cumbersome/expensive than MRI scanners, b) does not generate any magnetic interference with metallic implants and medical accessories, and c) subjects patients to significantly less radiation than traditional CT scanners, thereby reducing cancer risks. 

\begin{itemize}
    \item Need for convexity; the complete absence of convex methods (to our knowledge) in biplanar X-ray based reconstruction is the key problem we address in this article
    \item Our contributions
    \begin{enumerate}
        \item Highly accurate convex method for marker/correspondence based reconstruction from biplanar X-ray
        \item A convex relaxation to initialise the pose and shape of objects from biplanar X-ray, based on silhouettes and a 3D template
    \end{enumerate}
\end{itemize}


+++++++


% The image formation model of \citep{cai2024radiative}, while impressive for realistic novel view synthesis of X-rays, is prohibitively cumbersome for the sole purpose of determining the projected silhouette of shapes. We are not interested in the relative opacity of the Gaussian pointcloud; instead, we desire merely two properties from our image formation model, namely, when rendered using such a model from any arbitrary viewing direction, all image points: 1) inside the shape silhouette should have intensity values as high as possible, and, 2) outside the shape silhouette should have intensity values as low as possible.

% We assume that $(\mathbf{C}_1, \mathbf{C}_2)$ casts a total of $(Q, R)$ rays through $\mathbf{V}$ which forms two rendered X-ray images $(\mathcal{I}_1, \mathcal{I}_2)$. These set of rays are given by $\{L_{1,q}, \forall q \in [1,Q]\}$ and $\{L_{2,r}, \forall r \in [1,R]\}$ for the cameras $\mathbf{C}_1$ and $\mathbf{C}_2$ (resp.). Each ray is defined by the tuple $(\mathbf{C}_1, \mathbf{d}_{1,q})$ and $(\mathbf{C}_2, \mathbf{d}_{2,r})$ for $\mathbf{C}_1$, $\mathbf{C}_2$ resp., where $\mathbf{d}_{1,q}, \mathbf{d}_{2,r} \in \mathbb{S}^2, \forall q, r$. For the $q$-th and $r$-th sight-line, we denote the image formation model as:
% \begin{equation}
% \label{eqn_img_basic}
%     \mathcal{I}_{1}(\mathbf{v}_{1,j}) = \sum_{j=1}^N e^{-\frac{1}{\sigma_j^2} \big(d(\mathbf{V}_j, L_{1,q})\big)^2},  \quad \mathcal{I}_{2}(\mathbf{v}_{2,j}) = \sum_{j=1}^N e^{-\frac{1}{\sigma_j^2} \big(d(\mathbf{V}_j, L_{2,r})\big)^2},
% \end{equation}
% \noindent where $d(\cdot, \cdot) \in \mathbb{R}_+$ gives the normalised, squared-distance between a point and a line and $\{\sigma_j\}$ is a weight. The point-to-line distance function $d$ is derived from the shortest L$_2$-distance of the deformed shape $\mathbf{R}\mathbf{Q}$ to the sightlines, which are uniquely defined by $(\mathbf{C}_1, \mathbf{d}_{1,q})$ or $(\mathbf{C}_2, \mathbf{d}_{2,r})$, and are computable for each point of the shape. For the $j$-th point, $d(\cdot, \cdot)$ can be expressed as:
% \begin{equation}\label{eqn_long_expr_1}
%     d(\mathbf{V}_j, L_{x,y}) = d(\mathbf{R}\mathbf{Q}_j, L_{x,y}) = \frac{1}{\kappa} \|(\mathbf{R}\mathbf{Q}_j - \mathbf{C}_x + \langle \mathbf{C}_x - \mathbf{R}\mathbf{Q}_j, \mathbf{d}_{x,y}\rangle \mathbf{d}_{x,y} )\|_2, ~\forall (x,y) \in \{(1,q), (2,r)\},
% \end{equation}
% \noindent where $\kappa$ is the largest diagonal of the mean shape. Mildly simplifying \cref{eqn_long_expr_1} leads to:
% \begin{equation}
%     \begin{gathered}
%         d(\mathbf{V}_j, L_{x,y}) = 
%          \frac{1}{\kappa}\left\lVert \begin{bmatrix} \big((\mathbf{d}_{x,y} \mathbf{d}_{x,y}^{\top} - \mathbbm{1}_3) \otimes \mathbf{1}_{1 \times 3} \big) 
%              \big( \mathbf{1}_{1 \times M} \otimes \mathbbm{1}_9 \big)  \\ (\mathbf{d}_{x,y} \mathbf{d}_{x,y}^{\top} - \mathbbm{1}_3) \mathbf{C}_x \end{bmatrix}^{\top} \mathrm{diag}\Bigg(\begin{bmatrix}
%              (\mathbf{1}_{1 \times 3} \otimes \mathbf{P}_{j,1}^{\top})^{\top} \\ \vdots \\ (\mathbf{1}_{1 \times 3} \otimes \mathbf{P}_{j,M}^{\top})^{\top} \\ (\mathbf{1}_{1 \times 3} \otimes \tilde{\mathbf{P}}_j^{\top})^{\top} \\ 1
%          \end{bmatrix}^{\top}\Bigg) \begin{bmatrix}
%              w_1 \mathrm{vec}(\mathbf{R}) \\ \vdots \\ w_M \mathrm{vec}(\mathbf{R}) \\ \mathrm{vec}(\mathbf{R}) \\ - 1
%          \end{bmatrix} \right\rVert_2  \\
%         = \frac{1}{\kappa} \| \mathbf{A}_{(x,y,j)} \xi_{s} \|_2 \quad \forall (x,y) \in \{(1,q), (2,r)\}.
%     \end{gathered}
% \end{equation}
% \noindent Here, $\mathbf{A}_{(x,y,j)} \in \mathbb{R}^{3 \times 1 + 10M}$ is a data term and $\xi_{s} \in \mathbb{R}^{1 + 10M}$ is a vector derived from $\mathbf{R}$ and $\{w_i\}$. While reconstructing $\mathbf{Q}$ from the silhouettes, $\xi_{s}$ encompasses all the unknowns and all elements of $\mathbf{A}_{(x,y,j)}$ are known. We can introduce two Gram matrices $\Delta_s = \xi_{s} \xi_{s}^{\top}$ and $\mathbf{G}_{(x,y,j)} = \mathbf{A}_{(x,y,j)}^{\top} \mathbf{A}_{(x,y,j)}$, allowing us to write $\big(d(\mathbf{V}_j, L_{x,y})\big)^2 = \frac{1}{\kappa} \langle \mathrm{vec}(\mathbf{G}_{(x,y,j)}), \mathrm{vec}(\Delta_s) \rangle$ for any $(x,y) \in \{(1,q), (2,r)\}$ and $j \in [1, N]$.

% Importantly, the projected silhouettes partition the input images into two sub-spaces $(\tilde{\mathbf{S}}_{x^+}, \tilde{\mathbf{S}}_{x^-}) \subset \mathbb{R}^2$ corresponding to the region of the image inside and outside the silhouette (resp.), for all $x \in \{1,2\}$. For S\textit{b}-S\textit{f}T, $(\tilde{\mathbf{S}}_{x^+}, \tilde{\mathbf{S}}_{x^-})$ is part of the input data. At this point, to help the discussion, we add another mild assumption to the silhouette formation model:
% \begin{assume}\label{assum_2}
%     The centroid of $\mathbf{Q}$ is sufficiently close to the centroid of the visual hull obtained from $\tilde{\mathbf{S}}_{1^-}$ and $\tilde{\mathbf{S}}_{2^-}$
% \end{assume}
% \noindent \Cref{assum_2} is less milder than \cref{assum_1}, but for convex shapes, it was recently shown that the difference between the centroid of projection and projection of centroid can be, at worst, 0.2016 the width of $\mathbf{Q}$ \citep{myroshnychenko2023far} for one view. For two-views, this worst-case error can only be lesser, and cannot exceed the worst-case for one view. Although no such guarantees exist for general non-convex shape. But nonetheless, \cref{assum_2} can be enforced easily by prescribing imaging directions based on the spectral properties of $\mathbf{Q}$.

% \textcolor{red}{To add stuff.. }
% \vspace{5mm}
% \begin{itemize}
%     \item Traditional Gaussian splatting has already been utilised by [xxx] to generate realistic X-rays in xxxx (\textcolor{red}{this should be in `previous work'})
%     \item We wish to simplify it
%     \item We assume that $(\mathbf{C}_1, \mathbf{C}_2)$ casts a total of $(Q, R)$ rays through $\mathbf{V}$ which forms two X-ray images $(\mathcal{I}_1, \mathcal{I}_2)$. These set of rays are given by $\{L_{1,q}, \forall q \in [1,Q]\}$ and $\{L_{2,r}, \forall r \in [1,R]\}$ for the cameras $\mathbf{C}_1$ and $\mathbf{C}_2$ (resp.). Each ray is defined by the tuple $(\mathbf{C}_1, \mathbf{d}_{1,q})$ and $(\mathbf{C}_2, \mathbf{d}_{2,r})$ for $\mathbf{C}_1$, $\mathbf{C}_2$ resp., where $\mathbf{d}_{1,q}, \mathbf{d}_{2,r} \in \mathbb{S}^2, \forall q, r$. For the $q$-th and $r$-th sight-line, we denote the image formation model as:
% \begin{equation}
% \label{eqn_img_basic}
%     \mathcal{I}_{1}(\mathbf{v}_{1,j}) = \sum_{j=1}^N e^{-\frac{1}{\sigma_j^2} \big(d(\mathbf{V}_j, L_{1,q})\big)^2},  \quad \mathcal{I}_{2}(\mathbf{v}_{2,j}) = \sum_{j=1}^N e^{-\frac{1}{\sigma_j^2} \big(d(\mathbf{V}_j, L_{2,r})\big)^2},
% \end{equation}
% \noindent where $d(\cdot, \cdot) \in [0,1]$ gives the normalised distance between a point and a line and $\{\sigma_j\}$ is a weight.
% \item \textbf{Proposition 1}: The silhouettes partition the input images into two sub-spaces $(\tilde{\mathbf{S}}_{x^+}, \tilde{\mathbf{S}}_{x^-}) \subset [-1,1]^2$ corresponding to the region of the image inside and outside the silhouette (resp.), for all $x \in \{1,2\}$.
% \item The distance function $d(\cdot, \cdot)$ can be expressed as the function:
% \begin{equation}
%     \begin{gathered}
%     \label{eqn_long_expr_1_xxx}
%         d(\mathbf{V}_j, L_{1,q}) = d(\mathbf{R}\mathbf{Q}_j, L_{1,q}) = \frac{1}{\Delta} \|(\mathbf{R}\mathbf{Q}_j - \mathbf{C}_1 + \langle \mathbf{C}_1 - \mathbf{R}\mathbf{Q}_j, \mathbf{d}_{1,q}\rangle \mathbf{d}_{1,q} )\|_2 \\
%          = \frac{1}{\Delta}\left\lVert \begin{bmatrix} \big((\mathbf{d}_{1,q} \mathbf{d}_{1,q}^{\top} - \mathbbm{1}_3) \otimes \mathbf{1}_{1 \times 3} \big) 
%              \big( \mathbf{1}_{1 \times M} \otimes \mathbbm{1}_9 \big)  \\ (\mathbf{d}_{1,q} \mathbf{d}_{1,q}^{\top} - \mathbbm{1}_3) \mathbf{C}_1 \end{bmatrix}^{\top} \mathrm{diag}\Bigg(\begin{bmatrix}
%              (\mathbf{1}_{1 \times 3} \otimes \mathbf{P}_{j,1}^{\top})^{\top} \\ \vdots \\ (\mathbf{1}_{1 \times 3} \otimes \mathbf{P}_{j,M}^{\top})^{\top} \\ (\mathbf{1}_{1 \times 3} \otimes \tilde{\mathbf{P}}_j^{\top})^{\top} \\ 1
%          \end{bmatrix}^{\top}\Bigg) \begin{bmatrix}
%              w_1 \mathrm{vec}(\mathbf{R}) \\ \vdots \\ w_M \mathrm{vec}(\mathbf{R}) \\ \mathrm{vec}(\mathbf{R}) \\ - 1
%          \end{bmatrix} \right\rVert_2  
%     \end{gathered}
% \end{equation}
% \item \textcolor{red}{New properties of silhouettes go here}
% \end{itemize}

+++++++++++



% We introduce the auxiliary variable $\mathbf{M}_j \in \mathbb{R}^3$ such that $\Pi(g_1(\mathbf{M}_j)) = \mathbf{p}_{1, \mathbf{q}}$ and $\Pi(g_2(\mathbf{M}_j)) = \mathbf{p}_{2, \mathbf{r}}$. $\mathbf{M}_j$ signifies the point where the line joining $\mathbf{C}_1$ to $\mathbf{p}_{1, \mathbf{q}}$ and $\mathbf{C}_2$ to $\mathbf{p}_{2, \mathbf{r}}$ intersect in space. Introducing $\mathbf{M}_j$ into \cref{eqn_pt_based} results in:
% \begin{equation}\label{eqn_pt_based_first_reparam}
%     \begin{gathered}
%         \min_{\mathbf{R}, \{w_i\}, \{\mathbf{M}_j\}} \sum_{(j, \mathbf{p}_{1,j_1}, \mathbf{p}_{2,j_2}) \in \Omega} \| \mathbf{V}_j - \mathbf{M}_j\|_1 , \\
%         \text{s.t.:} \quad \mathbf{V}_j = \mathbf{R}\Big(\bar{\mathbf{P}}_j + \sum_{i=1}^M w_i \mathbf{P}_{i,j}\Big), \quad \Pi(g_1(\mathbf{M}_j)) = \mathbf{p}_{1, \mathbf{q}}, \quad \Pi(g_2(\mathbf{M}_j)) = \mathbf{p}_{2, \mathbf{q}},
%         ~ \mathbf{R} \in \mathbb{SO}(3) .
%      \end{gathered}
% \end{equation}
% \noindent There exists, necessarily, an unique set of points $\{\mathbf{M}_j\}$, since no parallel lines between any two lines of $\{L_{1,r}\}$ and $\{L_{2,q}\}$ can belong to the correspondence set $\Omega$. Therefore, the lines joining $\mathbf{C}_1$ to $\mathbf{p}_{1, \mathbf{q}}$ and $\mathbf{C}_2$ to $\mathbf{p}_{2, \mathbf{r}}$ either: 1) perfectly intersect each other in $\mathbb{R}^3$ if the correspondences are noiseless, or 2) more realistically, do not intersect but are not parallel either. In this second case of noisy correspondences, one can estimate the point closest to both the lines, which forms the best estimate of $\mathbf{M}_j$. \textcolor{blue}{Check appendix}. Therefore, $\{\mathbf{M}_j\}$ can be estimated independently of $\mathbf{R}$ and $\{w_i\}$ by solving the feasibility problem:
% \begin{equation}\label{eqn_pt_feasibility}
%     \begin{gathered}
%         \min_{\{\mathbf{M}_j\}} 0 , \\
%         \text{s.t.:} \quad \Pi(g_1(\mathbf{M}_j)) = \mathbf{p}_{1, \mathbf{q}}, \quad \Pi(g_2(\mathbf{M}_j)) = \mathbf{p}_{2, \mathbf{q}}, \quad \forall (j, \mathbf{p}_{1,j_1}, \mathbf{p}_{2,j_2}) \in \Omega,
%      \end{gathered}
% \end{equation}
% \noindent or a dual of the problem in \cref{eqn_pt_feasibility}, if noisy correspondences makes the primal infeasible. Importantly, reprojective constraints as in \cref{eqn_pt_feasibility} are linear and a global optima can be easily achieved in the linear least squares sense. With a slight abuse of notation, we now consider $\Omega$ to have only those indices ($j$) for which a corresponding $\mathbf{M}_j$ has been estimated. Assuming $\{\tilde{\mathbf{M}}_j\}$ to be the optimal solution of \cref{eqn_pt_feasibility}, we plug it back into \cref{eqn_pt_based_first_reparam}, giving us:
% \begin{equation}\label{eqn_pt_based_second_reparam}
%     \begin{gathered}
%         \min_{\mathbf{R}, \{w_i\}} \sum_{j \in \Omega} \| \mathbf{V}_j - \tilde{\mathbf{M}}_j\|_1 , \\
%         \text{s.t.:} \quad \mathbf{V}_j = \mathbf{R}\Big(\bar{\mathbf{P}}_j + \sum_{i=1}^M w_i \mathbf{P}_{i,j}\Big),\quad \forall~j\in\Omega, \quad \mathbf{R} \in \mathbb{SO}(3).
%      \end{gathered}
% \end{equation}
% \noindent \Cref{eqn_pt_based_second_reparam} is still non-convex due to the special orthogonality requirements of $\mathbf{R}$. We use the Shor's relaxation to linearise the rotational constraints. We introduce the parameter vector $\xi_p = (1, \mathrm{vec}(\mathbf{R})^{\top}, w_1, \hdots, w_M)^{\top}$ and the Gram matrix $\Delta_p = \xi_p \xi_p^{\top}$ which is positive semi-definite by construction. This allows us to write \cref{eqn_pt_based_second_reparam} as the following SDP problem:
% \begin{equation}\label{eqn_pt_based_final}
%     \begin{gathered}
%         \min_{\Delta_p} \sum_{j \in \Omega} \| \mathrm{tr}\Big(\omega_1(j) \Delta_p\Big) - \tilde{\mathbf{M}}_j\|_1 , \\
%         \text{s.t.:} \quad \Delta_p \in \mathcal{S}_+^{10+M},~  \mathrm{tr}\Big(\theta_y \Delta_p\Big)  = 0, ~\forall y \in [1,15],
%      \end{gathered}
% \end{equation}
% where $\{\theta_y\}$ corresponds to the fifteen rotational constraints arising out of the requirements of $\mathbb{SO}(3)$, i.e., $\mathbf{R}\mathbf{R}^{\top} - \mathbbm{1}_3 = 0$ and $\text{det}(\mathbf{R}) = 1$. Please check appendix \textcolor{blue}{[xxx]} for the details of $\omega_1$ and $\{\omega_y\}$. 


+++++

\vspace{10mm}
\subsection{Silhouette-based shape-from-template for biplanar X-rays}\label{silh_based}
\textcolor{red}{To be completely modified...}

The key challenge for S\textit{b}-S\textit{f}T is the absence of correspondence. The silhouette information, supplied in the form of $(\tilde{\mathbf{S}}_{x^+}, \tilde{\mathbf{S}}_{x^-})$ for $x \in \{1,2\}$ splits the input image into regions within and outside the silhouette. We denote by $\big\{L_{x,y^+}, \forall (x,y) \in \{(1,q), (2,r)\}\big\}$, the $M_x$ sightlines that intersect the images outside the silhouettes.
%The silhouette bisects the input data into two sub spaces, $\tilde{\mathcal{I}}_{1,q^+}$, $\tilde{\mathcal{I}}_{2,r^+}$ for the 2D points outside the silhouette and $\tilde{\mathcal{I}}_{1,q^-}$, $\tilde{\mathcal{I}}_{2,r^-}$ for the keypoints inside the silhouette.

\subsubsection{Problem statement.} The key idea for S\textit{b}-S\textit{f}T is to ensure that the projected image of the deformed shape never falls into $\{L_{x,y^+}\}$. This can be ensured by minimising the intensity along all the sightlines lying outside the silhouette, for both the cameras. Therefore, the problem we want to solve is the following:
\begin{equation}\label{silh_based_prblm_stmt}
   \boxed{ \begin{gathered}
        \min_{\mathbf{R}, \{w_i\}} \sum_{q^+ = 1}^{M_1}\sum_{j=1}^N e^{-\frac{1}{\sigma_j^2} \big(d(\mathbf{V}_j, L_{1,q^+})\big)^2} + \sum_{r^+ = 1}^{M_2}\sum_{j=1}^N e^{-\frac{1}{\sigma_j^2} \big(d(\mathbf{V}_j, L_{2,r^+})\big)^2} \\
        \text{s.t.:}~\mathbf{R} \in \mathbb{SO}(3), ~\mathbf{V}_j = \mathbf{R}\Big(\bar{\mathbf{P}}_j + \sum_{i=1}^M w_i \mathbf{P}_{i,j}\Big)
    \end{gathered}}
\end{equation}
\subsubsection{Solution.} We have two sources of non-linearity in \cref{silh_based_prblm_stmt}: 1) the polynomials in the exponent of the exponential terms in the cost, and 2) the rotational constraints themselves. Both these problems can be easily solved with Shor's relaxation. We utilise the $\Delta_s = \xi_s \xi_s^{\top}$ introduced in \cref{silh_formation_model} for the SDP formulation. Notice that $\xi_s$ has redundant repetitions of the elements of $\mathbf{R}$. Therefore, we reparameterise the variables
\begin{equation}
    \xi_s = (\mathrm{vec}(\boldsymbol{\gamma})^{\top}, \mathrm{vec}(\mathbf{R})^{\top}, -1)^{\top}, \quad \text{where,} \quad \boldsymbol{\gamma} = \big(\mathbf{w}^{\top} \otimes \mathrm{vec}(\mathbf{R})^{\top}\big)^{\top}, \quad \text{and}, \quad \mathbf{w} = \big( w_1, \hdots, w_M \big)^{\top},
\end{equation}
into a vector $\xi_h$ with seperate terms for each product of monomials, i.e., 
\begin{equation}
    \xi_h = \big( \boldsymbol{\gamma}_{h}^{\top},\mathrm{vec}(\mathbf{R})^{\top}, -1 \big)^{\top} \qquad \text{where} \qquad \boldsymbol{\gamma}_{h} = \big(\boldsymbol{\gamma}_{h,1}, \hdots, \boldsymbol{\gamma}_{h, 9M}\big)^{\top} \in \mathbb{R}^{9M}.
\end{equation}
This leads to a new Gram matrix $\Delta_h = \xi_h\xi_h^{\top}$. Notice that there are redundant terms in $\xi_s$, which must be converted to constraints in any optimisation parameterised by $\xi_h$ or $\Delta_h$, e.g.: the relation $\frac{w_1 r_{1,1}}{r_{1,1}} = \frac{w_1 r_{1,2}}{r_{1,2}}$ in the elements of $\xi_s$ converts to the constraint $\boldsymbol{\gamma}_{h,1} r_{1,2} - \boldsymbol{\gamma}_{h,2} r_{1,1} = 0$ in $\xi_h$. In the POP literature, there exists the notion of \textit{moment constraints} \citep{henrion2009gloptipoly, lasserre2009moments} which constrains redundant terms inside these Gram matrices. We use a variant of such moment constraints to constrain the redundant terms in $\Delta_h$. Exactly $8M$ such constraints on the elements of $\Delta_h$ are sufficient to account for all elements of the rotation matrix, i.e.,
\begin{equation}\label{mom_cons}
    \Delta_{h,1,9l - 8} \Delta_{h,1,9M + m} - \Delta_{h,1,9l+m-9} \Delta_{h,1,9M+1} = 0, \quad \forall  l \in [1,M], ~m \in [2,9].
\end{equation}
\noindent \Cref{mom_cons} can be expressed as $\mathrm{tr}(\psi_{x} \Delta_h)$, with some suitable sampling operator $\psi_{x}$. Therefore, we can reformulate \cref{silh_based_prblm_stmt} into the following SDP problem:
\begin{equation}\label{silh_based_first}
    \begin{gathered}
        \min_{\Delta_h} \sum_{q^+ = 1}^{M_1}\sum_{j=1}^N e^{-\frac{\mathrm{tr}\big(\omega_2(j, q^+) \Delta_h\big)}{\sigma_j^2} } + \sum_{r^+ = 1}^{M_2}\sum_{j=1}^N e^{-\frac{\mathrm{tr}\big(\omega_2(j, r^+) \Delta_h\big)}{\sigma_j^2}} \\
        \text{s.t.:}\quad \Delta_h \in \mathcal{S}_+^{10+M},~  \mathrm{tr}\big(\psi_{x} \Delta_h\big)  = 0,~ \text{and}~  \mathrm{tr}\big(\hat{\theta}_{y} \Delta_h\big)  = 0, ~\forall x \in [1,8], ~y \in [1,15].
    \end{gathered}
\end{equation}
\noindent $\hat{\theta}_{y}$ are the sampling matrices corresponding to the constraints of $\mathbb{SO}(3)$ derived from $\Delta_h$. \Cref{silh_based_first} is already convex, solvable by standard ECP. One might assume the problem to be solved well enough at this stage; however, unfortunately, this is not the case. 

\vspace{2mm}
\noindent \textbf{Escape to higher rank}. The solution in \cref{silh_based_first} often produces an optimal $\tilde{\Delta}$ that is high-rank, i.e., $\mathrm{rank}(\tilde{\Delta}) > 1$. This is a known and well-studied pitfall \citep{brynte2022tightness} of many SDP-based solutions of popular problems in geometric perception; in our case, the rank relaxation happens due to : 1) ill-posedness of the primal cost in \cref{silh_based_first} due to very large and small values of $\{\sigma_j\}$, and 2) the linearised rotational constraints $\{\omega_y(j)\}$ exacerbates the problem, often making low-rank solutions infeasible.

We propose to solve this problem by, starting from the relaxed solution $\tilde{\Delta}$, \textit{first} projecting the rotational component of $\tilde{\Delta}$ into the rotation manifold, and \textit{second}, optimising alternately for rotations and shape basis weights separately following a block relaxation paradigm \citep{de1994block}, each optimisation of rotation being followed by repeated optimal projection into the rotation manifold. The overall idea combines the optimal metric projection approach with block relaxation, applied to \cref{silh_based_first} to produce two alternating optimisation. The detailed description follows. 

\vspace{2mm}
\noindent \textbf{Optimal metric projection}. Projection of $\tilde{\Delta}$ to the rotation manifold involves three operations: 1) projection of $\tilde{\Delta}$ to the rank-1 manifold, we denote this operation by the function $Pr_{\mathrm{rank}}$, 2) extracting the putative rotation matrix from the rank-1 Gram matrix, we denote this operation by the function $\varphi$, 3) projecting the putative rotation matrix to the nearest point on the rotation manifold, we denote this operation by the function $Pr_{\mathbb{SO}(3)}$. The combined mechanism to project $\tilde{\Delta}$ to the rotation manifold, denoted by the function $Pr_{\mathrm{opt}}$, is therefore a composition of these three functions:
\begin{equation}
    Pr_{\mathrm{opt}} = Pr_{\mathbb{SO}(3)} \circ \varphi \circ Pr_{\mathrm{rank}}
\end{equation}

We now briefly describe $Pr_{\mathrm{rank}}$, $\varphi$, and $Pr_{\mathbb{SO}(3)}$, all of which follow standard methods. $Pr_{\mathrm{rank}}$ finds the nearest rank-1 matrix to $\tilde{\Delta}$, say $\tilde{\Delta}_1$, by discarding all but the highest singular value, i.e., $ \tilde{\Delta}_1 = Pr_{\mathrm{rank}}(\tilde{\Delta}) = \mathbf{U}_{\Delta} \mathbf{D}_{\Delta,1,1} \mathbf{V}_{\Delta}$, where $\mathbf{U}_{\Delta}\mathbf{D}_{\Delta}\mathbf{V}_{\Delta} = \mathrm{svd}(\tilde{\Delta})$. $\varphi$ uses another round of SVD decomposition of $\tilde{\Delta}_1$ to retrieve the putative rotation matrix $\tilde{\mathbf{R}}$, therefore $ \mathrm{vec}(\tilde{\mathbf{R}}) = \varphi(\tilde{\Delta}_1) = \mathbf{U}_{\Delta_1} \sqrt{\mathbf{D}_{\Delta_1,1,1}}$, where $\mathbf{U}_{\Delta_1}\mathbf{D}_{\Delta_1}\mathbf{V}_{\Delta_1} = \mathrm{svd}(\tilde{\Delta}_{1, 10 \times 10})$, where $\tilde{\Delta}_{1, 10 \times 10}$ is the lower-right $10 \times 10$ sub-matrix of $\tilde{\Delta}_1$ (corresponding to the rotational components). However, the action of $\varphi \circ Pr_{\mathrm{rank}}$ on $\tilde{\Delta}$ may cause some of the rotational constraints to be violated. Therefore, with $Pr_{\mathbb{SO}(3)}$, we use the well-known Cayley's method \citep{sarabandi2019cayley} for projecting $\tilde{\mathbf{R}}$ to the nearest point on the rotation manifold. We denote by $\tilde{\mathbf{R}}_0$ and $\{\tilde{w}_{i,0}\}$, the projected rotation matrix and basis weights recovered by the action of $Pr_{\mathrm{opt}}$ on $\tilde{\Delta}$.

\vspace{2mm}
\noindent \textbf{Block relaxation}. To obtain a sufficiently low-rank solution to the problem in \cref{silh_based_prblm_stmt}, we refine the relaxed results from the convex solution in \cref{silh_based_first} by two rounds of iterative parameter-wise block relaxation. The two rounds of relaxations are: 1) \textit{first}, we split the optimisation parameter into two separate optimisations, one for the rotational component $\mathbf{R}$ and another for the basis weights $\{w_i\}$, we denote this first round by $\text{BR}_1$, 2) \textit{second}, we split the optimisation for the rotation into optimisation for 3 separate $2 \times 2$ sub-matrices, we denote this first round by $\text{BR}_2$. We now describe these two set of relaxations in detail.

\vspace{2mm}
\noindent \textbf{$\text{BR}_1$}. We split the optimisation into rotation and shape bases weights. For rotation, we denote by $\Delta_{\mathbf{R}} = \xi_{\mathbf{R}} \xi_{\mathbf{R}}^{\top}$, the Gram matrix of rotation from $\xi_{\mathbf{R}} = (1, \mathrm{vec}(\mathbf{R})^{\top})^{\top}$. At the $t$-th iteration of $\text{BR}_1$, we denote the last known estimate of basis weights as $\{w_{i,t}\}$, where $\{w_{i,0}\}$ is recovered by the action of $Pr_{\mathrm{opt}}$ on $\tilde{\Delta}$. With this estimate, we solve for rotation via the first sub-problem:
\begin{equation}\label{silh_based_rot}
    \begin{gathered}
        \min_{\Delta_{\mathbf{R}}} \sum_{q^+ = 1}^{M_1}\sum_{j=1}^N e^{-\frac{\mathrm{tr}\big(\omega_3(j, q^+, \{w_{i,t}\}) \Delta_{\mathbf{R}}\big)}{\sigma_j^2} } + \sum_{r^+ = 1}^{M_2}\sum_{j=1}^N e^{-\frac{\mathrm{tr}\big(\omega_3(j, r^+, \{w_{i,t}\}) \Delta_{\mathbf{R}}\big)}{\sigma_j^2}} \\
        \text{s.t.:}\quad \Delta_{\mathbf{R}} \in \mathcal{S}_+^{10},~ \text{and}~  \mathrm{tr}\Big(\theta_y^{\ast} \Delta_{\mathbf{R}} \Big)  = 0, ~\forall y \in [1,15].
    \end{gathered}
\end{equation}
\noindent ${\theta}_{y}^{\ast}$ are the sampling matrices corresponding to the constraints of $\mathbb{SO}(3)$ derived from $\Delta_{\mathbf{R}}$. Ideally, if \cref{silh_based_rot} produces low-rank solutions, $\tilde{\mathbf{R}}_0$ could have been discarded. Unfortunately, \cref{silh_based_rot}, while tighter than \cref{silh_based_first}, still produces high rank solutions (but not full rank), requiring some further relaxations before sufficiently low-rank solutions emerge. Therefore, for just the rotations, we propose the second round of relaxation, described later in $\text{BR}_2$. 

At the $t$-th iteration of $\text{BR}_1$, we denote the last known estimate of rotation as $\mathbf{R}_t$. Therefore, the second sub-problem of $\text{BR}_1$ is:
\begin{equation}\label{silh_based_wt}
    \begin{gathered}
        \min_{\{w_i\}} \sum_{q^+ = 1}^{M_1}\sum_{j=1}^N e^{-\frac{1}{\sigma_j^2} \big(d(\mathbf{V}_j, L_{1,q^+})\big)^2} + \sum_{r^+ = 1}^{M_2}\sum_{j=1}^N e^{-\frac{1}{\sigma_j^2} \big(d(\mathbf{V}_j, L_{2,r^+})\big)^2} \\
        \text{s.t.:}~\mathbf{V}_j = \mathbf{R}_t\Big(\bar{\mathbf{P}}_j + \sum_{i=1}^M w_i \mathbf{P}_{i,j}\Big)
    \end{gathered}
\end{equation}
\noindent Note that \cref{silh_based_wt} is already linear in terms of $\{w_i\}$, therefore we managed to discard the SDP formulation and directly obtain \cref{silh_based_wt} from the original formulation of \cref{silh_based_prblm_stmt}.

\vspace{2mm}
\noindent \textbf{$\text{BR}_2$}. The next round of relaxations are in the elements of the rotation matrix. We utilise three sub-matrices of rotation matrix, $\mathbf{R}_{[1,1]}$, $\mathbf{R}_{[2,2]}$, and $\mathbf{R}_{[3,3]}$, defined as:
\begin{equation}
    \mathbf{R} = \begin{pmatrix}
        r_{1,1} & r_{1,2} & r_{1,3}\\
        r_{2,1} & r_{2,2} & r_{2,3}\\
        r_{3,1} & r_{3,2} & r_{3,3}
    \end{pmatrix}, \quad \mathbf{R}_{[1,1]} = \begin{pmatrix}
        r_{1,1} & r_{1,2}\\
        r_{2,1} & r_{2,2}\\
    \end{pmatrix}, \quad \mathbf{R}_{[2,2]} = \begin{pmatrix}
        r_{1,1} & r_{1,3}\\
        r_{3,1} & r_{3,3}
    \end{pmatrix}, \quad \mathbf{R}_{[3,3]} = \begin{pmatrix}
        r_{2,2} & r_{2,3}\\
        r_{3,2} & r_{3,3}
    \end{pmatrix}.
\end{equation}
\noindent At each step of the relaxation, for the elements of the rotation matrix which are not part of the parameter, we use the values from the last estimate as a prior. E.g.: when optimising for $\mathbf{R}_{t,[1,1]}$, the values of $r_{1,3}$, $r_{2,3}$, $r_{3,1}$, $r_{3,2}$, and $r_{3,3}$ are mandated to be close to their respective values in $\mathbf{R}_{t-1,[1,1]}$. We denote the vector of elements left out from $\mathbf{R}_{[z,z]}, ~\forall z \in [1,3]$ as $\mathbf{R}'_{[z,z]}$. Therefore, the iterative update, for the $z$-th rotation block is:
\begin{equation}
    \begin{gathered}
        \min_{\Delta_{\mathbf{R}_{t,[z,z]}}, \mathbf{R}'_{t,[z,z]}}  \sum_{q^+ = 1}^{M_1}\sum_{j=1}^N e^{-\frac{\mathrm{tr}\big(\omega_4(j, q^+, \{w_{i,t}\},\mathbf{R}'_{t,[z,z]}) \Delta_{\mathbf{R}_{t,[z,z]}}\big)}{\sigma_j^2} } + \sum_{r^+ = 1}^{M_2}\sum_{j=1}^N e^{-\frac{\mathrm{tr}\big(\omega_4(j, r^+, \{w_{i,t}\},\mathbf{R}'_{t,[z,z]}) \Delta_{\mathbf{R}_{t,[z,z]}}\big)}{\sigma_j^2}} \\ + \lambda \| \mathbf{R}'_{t,[z,z]} - \mathbf{R}'_{t-1,[z,z]} \|_2 \qquad
        \text{s.t.:}\quad \Delta_{\mathbf{R}_{t,[z,z]}} \in \mathcal{S}_+^{5},~ \text{and}~  \mathrm{tr}\Big(\tilde{\theta}_y \big(\Delta_{\mathbf{R}_{t,[z,z]}}, \mathbf{R}'_{t,[z,z]} \big) \Big)  = 0, ~\forall y \in [1,5].
    \end{gathered}
\end{equation}
\noindent where $\tilde{\theta}_y$ is the sampling matrix for rotational constraints in $\mathbb{SO}(2)$ and $\lambda \in (0, 10^{-3}]$ is a tunable parameter.


+++++++++++++


% We refer the readers to \citep{anjos2011handbook} for an overview of algebraic geometry and the various SDP-based solutions to the Polynomial Optimisation Problem (POP). We demonstrate a toy example as follows: to minimise a S\textit{o}S polynomial $f(\mathbf{R}, \textit{A})$, where $\mathbf{R} \in \mathbb{SO}(n)$ is a rotation matrix and $\textit{A}$ is a data term, the following optimisation:
% \begin{equation}\label{example_rot_min}
%     \min_{\mathbf{R}} f(\mathbf{R}, \textit{A}) ~\text{s.t.:}~\mathbf{R} \in \mathbb{SO}(n)
% \end{equation}
% \noindent can be posed as the equivalent SDP problem:
% \begin{equation}\label{eqn_shors}
%     \min_{\Delta} g_1(\Delta, \textit{A}), ~\text{s.t.:}~\Delta \in \mathcal{S}_+^{1 + n^2}, ~g_2(\Delta) = 0.
% \end{equation}
% \noindent This is possible by considering $\Delta = \big(1 ~\text{vec}(\mathbf{R})^{\top}\big)^{\top}\big(1~\text{vec}(\mathbf{R})^{\top}\big)$ as a Gram matrix, the terms in $f(\mathbf{R}, \textit{A})$ can now be expressed as a linear combination of the elements of $\Delta$, resulting in the new function $g_1(\cdot, \cdot)$. The new constraint $g_2(\Delta)$ expresses the constraint $\mathbf{R} \in \mathbb{SO}(n)$ in terms of the elements of $\Delta$, all expressions being linear.

++++


% The only convex methods for S\textit{b}-S\textit{f}T utilise matchable textures \citep{prasad2005fast, menudetmodel} between the template and the image, which is difficult to obtain in many cases, especially in the context of biplanar X-rays. Moreover, when correspondences are actually available, we benefit from the availability of much more robust and efficient standard S\textit{f}T algorithms, making the silhouette information redundant. Therefore, when only silhouette information is available, there exists a strong necessity to find a method that initialises the pose to some global optima in a principled manner. Unfortunately, such a problem is highly ill-posed and suffer from multiple ambiguous global minima. But thankfully, given a known template, such ambiguities can be pre-determined, therefore an ambiguous solution can also be useful. But nonetheless, determining globally optimal S\textit{b}-S\textit{f}T without any correspondences is a difficult and yet unsolved problem. 

++++


% or to assume inter-image stereo correspondences allowing the utilisation of rigid epipolar constraints between views (since in simultaneous imaging from multiple cameras, the object is rigid between views). Indeed, with large number of correspondences, it is sufficient to solve \y{sft} separately in each view and determine the camera pose as an aposteriori step. However, in this article, we show that such an assumption about solvability of multi-view \y{sft} and camera pose problem via a two step solution of first solving \y{sft} and then estimating camera poses does not hold when the number of correspondences start to dwindle. 
% Therefore, to solve multi-view \y{sft} and camera pose with few correspondences, we introduce the generalised camera model to the multi-view setup. The generalised camera model assumes that the line joining the camera centre with the normalised keypoint in Euclidean space, i.e., the \y{sl}, does not necessarily intersect or obey parallelism for every keypoint. Unsurprisingly, such a generalisation brings some new challenges, mainly due to the large number of unknown camera poses. In this article, we handle this challenge and propose methods to solve this multi-view \y{sft} and pose problem, which we call the \y{nsc} problem, in a concise and convex formulation. 

% As an additional step, we show that when the silhouette information is available as input and if the cameras are perspective, it is possible to refine the solution to the \y{nsc} problem while considering the silhouette information jointly to arrive at a very accurate solution for highly deformed, complex shapes. \textcolor{blue}{To talk about learned priors}

++


%But traditional \y{p3p} involves the solution of a quartic equation which can have multiple or no solutions, depending on the input data \cite{haralick1994review}. \textcolor{blue}{This is one of the reasons why it makes practical and theoretical sense to try and utilise multiple cameras, hence the generalised camera}, to solve the problem. 

++


% The problem of non-rigidly registering the 3D template of an object to some observed information from a camera, also know as the \y{sft} problem, is considered solved [xxx] when a large number of accurate keypoint correspondences between the template and the image are available. However, problem arises when these keypoint correspondences are either a few or noisy or both. In such a setup with a few noisy correspondences, the need arises to utilise additional information, going beyond keypoint correspondences, to ensure accuracy of \y{sft}. Solving \y{sft} with fewer and/or noisier correspondences has wide-ranging applications starting from improved motion capture, marker-based \y{ar} to 3D reconstruction from radiography. In this article, we propose methods for \y{sft} that not only delivers reconstruction with few correspondences that is more accurate than the comparable state-of-the-art, but also utilises additional visual cues to boost the accuracy of reconstruction even further.

% We propose two additional visual cue to boost the accuracy of \y{sft} when keypoint correspondences are unreliable: the \textit{first} additional cue is the multi-view \y{sft} setup, wherein we consider the case of an object being imaged from multiple viewpoints with correspondences to a single 3D template but no correspondences between images, and the \textit{second} additional cue are the silhouettes of the objects being imaged. Indeed, the multi-view \y{sft} setup and the silhouettes form the most obvious geometric cues to boost the accuracy of \y{sft}. Many authors have utilised the photometric information of images for \y{sft} [xxxxx], but such photometric approaches tend to be inconsistent under dynamic lighting and does not generalise well between surface-based and volumetric reconstruction, e.g.: image formation model of colour cameras are radically different from similar models for medical imaging setup such as radiography; on the other hand, correspondences, pose information between multiple views and silhouettes remain consistent between all such imaging modalities. 

% Silhouettes has been widely used in literature [xxx] either as the sole information used for \y{sft} or rigid localisation, or in conjunction with keypoint correspondences. The multi-view \y{sft} setup is a less frequent variant of \y{sft}. Indeed, when correspondences are available between images, the problem can also be posed as classical \y{sfm} problem [xxx], and if the extrinsics between the views are known as well, the problem can be posed as the classic triangulation problem [xxxx] in computer vision. 

% ....

% The classical one-view \y{sft} is contained as one particular case of \y{nsc}. Importantly, \y{nsc} is distinct from solving $P$ different one-view \y{sft} problems, since \y{nsc} is aided by the additional rigidity constraint between views. Of course \y{nsc} can be considered with additional information such as silhouettes or known extrinsics between views; we explore and solve all these variants in this article. 

% \vspace{2mm}
% \noindent \textbf{Motivation}. There are many utilities for \y{nsc} and its variants. Indeed, medical imaging applications such 3D reconstruction from radiography is an important motivation. The standard method for 3D imaging of human anatomical features are either CT or MRI scan. But MRI and CT scanners, despite being highly accurate, suffers some well-known drawbacks. MRI scanners lack adequate portability and poses safety hazards for patients with implants, external devices and accessory medical devices due to the strong magnetic field it generates. CT scans subject patients to a high dosage of radiation due to repeated scans with X-rays. Large-scale surveys have highlighted an `inordinately (sic) increase in cancer risks' \citep{cao2022ct} from CT scans. Biplanar X-rays, on the other hand, work by simultaneously imaging anteroposterior and lateral views of the object to be reconstructed \citep{melhem2016eos}. Imaging from just two views in this biplanar setup, therefore, offer an attractive alternative to CT and MRI scans because: a) they are less cumbersome/expensive than MRI scanners, b) does not generate any magnetic interference with metallic implants and medical accessories, and c) subjects patients to significantly less radiation than traditional CT scanners, thereby reducing cancer risks. \textcolor{red}{ add motion capture...}

% \vspace{2mm}
% \noindent\textbf{Contributions.} A common strategy for modelling deformable objects is to restrict the deformations to a shape space using \y{ssm}, solutions to the \y{sft} problem with \y{ssm}s have indeed been explored in the context of motion capture with orthographic projections [xxx], our \textit{first} contribution therefore is to extend \y{ssm} based \y{sft} to perspective cameras with a new convex relaxation approach that beats the state-of-the-art methods in terms of accuracy. \textit{Secondly}, we extend this convex solution to the classical \y{sft} problem to the \y{nsc} problem, which is again a convex solution. \textit{Third}, we demonstrate a method to utilise the silhouette information, when available, with an iterative approach with a step-wise convex solution.

% \textcolor{red}{The following needs to be semi-formally introduced in the introduction:
% \begin{itemize}
%     \item \y{sl}
%     \item  Generalised projection
% % \end{itemize}}

% \hline
% \vspace{20mm}

++++


% \begin{lemma}\label{lemma_minimal}
%     Given there exists a 3D template $\mathbf{V}$ with correspondences to a 2D image $\mathcal{I}_1$ and to solve the \y{sft} problem, the \y{mnc} is $\psi$. To this \y{sft} problem, if $(P-1)$ other images are added in an \y{nsc} setup following \cref{defn_nsc} but with no inter-image stereo correspondence and for the combined \y{nsc} problem, let the \y{mnc} be $\psi'$, then necessarily:
%     \begin{equation}\label{min_no_corr}
%         \psi' = \max(\psi, 3P).
%     \end{equation}
% \end{lemma}
% \begin{proof}
% If any camera has less than 3 correspondences, its pose cannot be uniquely localised, therefore $3P$ total correspondence is a minimum requirement, exceeded only if $\psi > 3P$.
% \end{proof}
% \noindent Note that \cref{lemma_minimal} is a necessary but not sufficient condition for solvability of \y{nsc}, however, it allows us to observe some important properties of the \y{nsc} setup.


+++++


% \subsection{Deformation model}
% We now utilise the \y{nsc}/\y{scc} problem setup to help guide our choice of a suitable deformation model for the template $\mathbf{V}$.

% \vspace{2mm}
% \noindent \textbf{The underlying rigidity}. If we hope to solve the \y{nsc}/\y{scc} problem in the case of SPV$_0$ + SC$_{\geq 3}$/SC$_{< 3}$/SC$_\emptyset$, an important consideration is to utilise the fact that the shape to be reconstructed has been observed with simultaneous images, i.e., irrespective of its deformation from the template, the shape is rigid between views. 


% \noindent \textbf{\y{sft}}. A common idea for \y{sft} is to model deformation of the 3D template in a shape space given by a \y{ssm}. Indeed, such \y{ssm} based approaches have been used in motion capture [xxx], \y{ar} [xxxx], medical imaging [xxxx], to name a few application areas. Recently, surface based \y{sft} [xxxx] approaches have gained popularity which utilises the known physics of deforming surfaces to constraint the motion of the template (c.f. \y{ssm}), however, not all objects have well defined surfaces, e.g.: articulated objects, volumetric objects with holes or any object imaged with X-rays. Nonetheless, when a well-defined surface exists, surface-based \y{sft} approaches have proven to be highly accurate [xxxx]. However, a key requirement of all prevalent \y{sft} methods are a large number of keypoint correspondences between the template and the image. Such a strong dependence on feature correspondences are problematic for two reasons: \rom{1}) Such keypoint correspondences are difficult to obtain in many applications and feature matching is susceptible to inaccuracies under challenging circumstances involving sudden lighting changes, motion blurs, occlusions, to name a few. \rom{2}) There exists many cases when there exists no matchable texture between the template and the image. Cases involving generic templates of objects are commonly known to be difficult to match with images [xxxx]. But there are even more challenging cases, e.g.: X-ray images in medical applications, where the textural appearance between the model and image are unrelated. For such medical applications, many learning based feature matchers [xxx] have been proposed recently, but the domain gap remains very high, preventing wide-spread usage. 
% \vspace{2mm}
% \noindent \textbf{Application specific methods}. Conceptually, the idea of optical camera based motion capture bears resemblance to many other applications. 


% % On the other hand, even for cases where feature matching is available, challenges exist when the matched correspondences are few and/or noisy [xxx]. Therefore, it is natural to seek methods to boost the accuracy of existing correspondence based \y{sft} methods. We review two approaches for improving the accuracy of \y{sft}: \rom) 


% \textcolor{red}{to write more...}

% \vspace{10mm}
% We now review some of the previous works on reconstructing 3D structure from biplanar X-rays in a clinical setup. There are two broad approaches for template-based reconstruction, one involves the presence of some correspondences between the template and the image and on the other hand, there are correspondence free approaches that use either the pre-identified shape silhouette or direct intensities of the X-rays. There exists a more challenging, template-free reconstruction from biplanar X-rays, all of which are based on deep learning, since just two-views are inadequate for accurate geometric reconstructions with classical approaches in all realistic cases.
% \vspace{2mm}
%  \noindent \textbf{Marker-based approaches}. For 2D markers with valid correspondences across images, two views represent the minimal setup required for an exact 3D triangulation. Naturally, a majority of 3D reconstruction methodologies from biplanar X-rays are marker based \citep{cheriet1999self, mitton20003d, pomero2004fast, nerot20153d,  gajny2019quasi, bousigues20233d, girinon2020quasi, baudoin2008parametric, laporte2003biplanar, baka_2d3d_2011}. Most of these approaches estimate the shape with the assumption of rigidity (e.g.: \citep{cheriet1999self, gajny2019quasi}), but many approaches also estimate the shape irrespective of deformations (e.g.: \citep{mitton20003d, nerot20153d}). To our knowledge, there still does not exist any biplanar X-ray based 3D reconstruction method that is based on convex optimisation.
%  \vspace{2mm}
%  \noindent \textbf{Marker-free approaches}. Attempts have been made in the direction of marker-free reconstruction from biplanar X-rays either based on shape-contour/silhouette information \citep{boussaid20113d, verstraete2017accuracy} or direct image intensities \citep{jecklin2022x23d, buttongkum20233d, van2022deep, kasten2020end}, but these methods solve the reconstruction problem in a non-convex formulation, thereby missing the much needed optimality guarantees which are highly desired in a clinical setup. The non-convex methods initialise their optimisation with some heuristic-based alignment (e.g.: PCA) and follow it up with iterative refinement steps. Such an approach is prone to local minima, especially since the initialisation is done heuristically from just two-views.
% \vspace{2mm}
%  \noindent \textbf{Learning-based reconstruction}. Recent approaches for template-free 3D reconstruction from biplanar X-rays have seen a boom in learning based approaches \citep{an2021robust, ying2019x2ct, shakya2023benchmarking, van2022deep, gao20233dsrnet, kyung2023perspective, chen2024automatic, cheng2023sdct}. But most of the available literature shows the importance of extensive domain specific training required for such reconstructions, e.g.: chest \citep{ying2019x2ct, cheng2023sdct, kyung2023perspective}, spine \citep{chen2024automatic, gao20233dsrnet}, femur \citep{van2022deep}, and cranium \citep{an2021robust}. Recent approaches such as \citep{shakya2023benchmarking} demonstrates how a wide variety of network architectures are all suited for the biplanar reconstruction problem but the tolerance for domain shift is limited to pathological cases and new population cohort within each category of shape, i.e., a new shape category requires re-training on large dataset with $>$~400 samples at least. Therefore, generalisation across the human anatomy remains challenging and infeasible in certain cases, when training samples are sparse.

%  \section{Background}
% When determining the shape and pose of an object from multiple calibrated perspective cameras with known extrinsics, the translation parameter of the model is trivially linear, leaving us with two important considerations: 1) parameterising rotations, and 2) defining and utilising the constraints imposed by the silhouette. We now present a brief background of how these two aspects have been classically handled in the existing literature, starting with \textit{rotations} in \cref{sec_rot} and \textit{silhouette} models and constraints in \cref{sec_silh}.
 
% \subsection{Parameterising rotations}\label{sec_rot}

 
%  \subsection{Silhouette representation}\label{sec_silh}



% \subsection{Multi-view \y{sft}}

% ...here is where we define \y{nsc}...
% Recent developments in the field of Exponential Cone Programming (ECP) \citep{chandrasekaran2017relative} has opened up many more opportunities for the advent of novel costs and constraints in geometric optimisation problems. ECP works within the same framework of SDP and can be utilised to solve problems when $f(\cdot, \cdot)$ in \cref{example_rot_min} involves exponential costs. This is interesting because recently, some authors began modifying Gaussian splatting techniques (see \citep{fei20243d} for a survey) for the purpose of novel view synthesis \citep{cai2024radiative} of X-rays. Specifically, \citep{cai2024radiative} formulates the X-ray image formation using a Gaussian pointcloud, where the radiation intensity of the centroid of each point is given by:
% \begin{equation}\label{GS_xray_init}
%     I(\mathbf{g}) = \frac{1}{1 + e^{\boldsymbol{\lambda}^{\top}\mathbf{g}}},
% \end{equation}
% where $\mathbf{g}$ is a learned feature vector and $\boldsymbol{\lambda}$ are constant weights. While the model proposed in \citep{cai2024radiative} is sufficiently sophisticated to meet the requirements of realistic X-ray image formation, there exists the opportunity that such an approach could be sufficiently simplified, especially when realistic images are not necessary, as in the case of silhouette generation, to fit the ECP problem structure.


% \begin{itemize}
%     \item Why metric matching is important for existing methods 
%     \item How Gaussian splatting could be a good candidate
%     \item First and second fundamental theorem of shape from silhouettes
% \end{itemize}


+++++


% We focus on the problem of \y{nsc} and explain its solution method, since it is the more challenging of the two

% We first describe the \y{nsc} problem setup \cref{prob_setup}. This is followed by the two problem statements addressed by us in this article: 1) the purely correspondence-based case of \y{nsc} in \cref{pt_based}, which includes its two sub-variants of with and without known extrinsics between the multiple views and 2) the silhouette-boosted \y{nsc} in \cref{silh_based}; the respective solution methodologies are provided following each problem statement.


++++


%The X-ray images are denoted by a map $\tilde{\mathcal{I}}_x : \mathbb{R}^2 \mapsto \mathbb{R}_+$ and $\mathcal{I}_x : \mathbb{R}^2 \mapsto \mathbb{R}_+$ for the input data and the modelled image (resp.). Additionally, we require as input, either \textit{point-correspondences} for S\textit{f}T, or \textit{object silhouette} for S\textit{b}-S\textit{f}T.


% \begin{itemize}
%     \item We assume that there are two X-ray cameras which are imaging a shape, the centre of these two cameras are at $\mathbf{C}_1, \mathbf{C}_2 \in \mathbb{R}^{3}$
%     \item The shape itself is $\mathbf{V} \in \mathbb{R}^{3 \times N}$ in object coordinates
%     \item The volumetric Statistical Shape Model (SSM) be represented by a 3D mean pointcloud of $N$ points denoted by $\bar{\mathbf{P}} \in \mathbb{R}^{3 \times N}$ and the basis pointcloud $\mathbf{P}_{i} \in \mathbb{R}^{3 \times N} \quad \forall i \in [1,M]$, where we have $M$ basis shapes. Assuming $\mathbf{R} \in \mathbb{SO}(3)$ to be the object to world coordinate rotation, the shape can be represented as:
% \begin{equation}
%     \mathbf{V} = \mathbf{R}\Big(\bar{\mathbf{P}} + \sum_{i=1}^M w_i \mathbf{P}_{i}\Big) = \mathbf{R} \mathbf{Q},
% \end{equation}
% where $\{w_i\}$ are the basis weights and $\mathbf{Q}$ is the deformed shape.
% \item The normalised images formed are $\{\mathbf{v}_1 \in \mathbb{R}^{2 \times N}\}$ and $\{\mathbf{v}_2 \in \mathbb{R}^{2 \times N}\}$, obtained with some known extrinsics $\Big( {}^{C_1}\mathbf{R}_{W} \in \mathbb{SO}(3), {}^{C_1}\mathbf{t}_{W} \in \mathbb{R}^3 \Big)$ and $\Big( {}^{C_2}\mathbf{R}_{W} \in \mathbb{SO}(3), {}^{C_2}\mathbf{t}_{W} \in \mathbb{R}^3 \Big)$ (resp.), i.e.,
% \begin{equation}
%         \mathbf{v}_x = \Pi \Big( {}^{C_x}\mathbf{R}_{W} \mathbf{V} +  {}^{C_x}\mathbf{t}_{W}\Big) = \Pi \big( g_x( \mathbf{V} )\big), \quad \forall ~x \in [1,2]
% \end{equation}
% \item The X-ray images are denoted by a map $\tilde{\mathcal{I}}_x : [-1,1]^2 \mapsto \mathbb{R}_+$ and $\mathcal{I}_x : [-1,1]^2 \mapsto \mathbb{R}_+$ for the input data and the modelled image (resp.)
% %; a 2D point $\mathbf{v}_{x,j} \in \mathbb{R}^2$ corresponds to a $q$-th point on $\mathcal{I}_x$/$\tilde{\mathcal{I}}_x$, where $q = \mathfrak{f}(\mathbf{v}_{x,j}) = W(\mathbf{v}_{x,j,1} - 1) + \mathbf{v}_{x,j,2}$ 
% \end{itemize}
+++


% use the newly proposed {\tt Bramante39M}\footnote{See supplementary materials for more details} as a data for the real, planar experiments. This dataset contains a piece of paper deforming across 9 configurations with 40 keypoint correspondences, each configuration has been captured from multiple viewpoints (between 6 and 10) and each image comes equipped with \y{gt} depths and camera pose. Three images of each configuration are also equipped with silhouettes. All data are in $m$.
